Enhancing Microgrid Performance Prediction with Attention-based Deep Learning Models

In this research, an effort is made to address microgrid systems' operational challenges, characterized by power oscillations that eventually contribute to grid instability. An integrated strategy is proposed, leveraging the strengths of convolutional and Gated Recurrent Unit (GRU) layers. This approach is aimed at effectively extracting temporal data from energy datasets to improve the precision of microgrid behavior forecasts. Additionally, an attention layer is employed to underscore significant features within the time-series data, optimizing the forecasting process. The framework is anchored by a Multi-Layer Perceptron (MLP) model, which is tasked with comprehensive load forecasting and the identification of abnormal grid behaviors. Our methodology underwent rigorous evaluation using the Micro-grid Tariff Assessment Tool dataset, with Root Mean Square Error (RMSE), Mean Absolute Error (MAE), and the coefficient of determination (r2-score) serving as the primary metrics. The approach demonstrated exemplary performance, evidenced by a MAE of 0.39, RMSE of 0.28, and an r2-score of 98.89\% in load forecasting, along with near-perfect zero state prediction accuracy (approximately 99.9\%). Significantly outperforming conventional machine learning models such as support vector regression and random forest regression, our model's streamlined architecture is particularly suitable for real-time applications, thereby facilitating more effective and reliable microgrid management.

==> mybibliography.tex <==
@inproceedings{cahuantzi2023comparison,
  title={A comparison of LSTM and GRU networks for learning symbolic sequences},
  author={Cahuantzi, Roberto and Chen, Xinye and G{\"u}ttel, Stefan},
  booktitle={Science and Information Conference},
  pages={771--785},
  year={2023},
  organization={Springer}
}
@article{wazirali2023state,
  title={State-of-the-art review on energy and load forecasting in microgrids using artificial neural networks, machine learning, and deep learning techniques},
  author={Wazirali, Raniyah and Yaghoubi, Elnaz and Abujazar, Mohammed Shadi S and Ahmad, Rami and Vakili, Amir Hossein},
  journal={Electric power systems research},
  volume={225},
  pages={109792},
  year={2023},
  publisher={Elsevier}
}
@inproceedings{cahuantzi2023comparison,
  title={A comparison of LSTM and GRU networks for learning symbolic sequences},
  author={Cahuantzi, Roberto and Chen, Xinye and G{\"u}ttel, Stefan},
  booktitle={Science and Information Conference},
  pages={771--785},
  year={2023},
  organization={Springer}
}
@inproceedings{cahuantzi2023comparison,
  title={A comparison of LSTM and GRU networks for learning symbolic sequences},
  author={Cahuantzi, Roberto and Chen, Xinye and G{\"u}ttel, Stefan},
  booktitle={Science and Information Conference},
  pages={771--785},
  year={2023},
  organization={Springer}
}
@inproceedings{pan2023hybrid,
  title={A hybrid quantum-classical approach based on the hadamard transform for the convolutional layer},
  author={Pan, Hongyi and Zhu, Xin and Atici, Salih Furkan and Cetin, Ahmet},
  booktitle={International Conference on Machine Learning},
  pages={26891--26903},
  year={2023},
  organization={PMLR}
}
@incollection{almeida2020multilayer,
  title={Multilayer perceptrons},
  author={Almeida, Luis B},
  booktitle={Handbook of Neural Computation},
  pages={C1--2},
  year={2020},
  publisher={CRC Press}
}
@article{wazirali2023state,
  title={State-of-the-art review on energy and load forecasting in microgrids using artificial neural networks, machine learning, and deep learning techniques},
  author={Wazirali, Raniyah and Yaghoubi, Elnaz and Abujazar, Mohammed Shadi S and Ahmad, Rami and Vakili, Amir Hossein},
  journal={Electric power systems research},
  volume={225},
  pages={109792},
  year={2023},
  publisher={Elsevier}
}
@article{gasparin2022deep,
  title={Deep learning for time series forecasting: The electric load case},
  author={Gasparin, Alberto and Lukovic, Slobodan and Alippi, Cesare},
  journal={CAAI Transactions on Intelligence Technology},
  volume={7},
  number={1},
  pages={1--25},
  year={2022},
  publisher={Wiley Online Library}
}
@article{hemeida2020nature,
  title={Nature-inspired algorithms for feed-forward neural network classifiers: A survey of one decade of research},
  author={Hemeida, Ashraf Mohamed and Hassan, Somaia Awad and Mohamed, Al-Attar Ali and Alkhalaf, Salem and Mahmoud, Mountasser Mohamed and Senjyu, Tomonobu and El-Din, Ayman Bahaa},
  journal={Ain Shams Engineering Journal},
  volume={11},
  number={3},
  pages={659--675},
  year={2020},
  publisher={Elsevier}
}
@article{sherstinsky2020fundamentals,
  title={Fundamentals of recurrent neural network (RNN) and long short-term memory (LSTM) network},
  author={Sherstinsky, Alex},
  journal={Physica D: Nonlinear Phenomena},
  volume={404},
  pages={132306},
  year={2020},
  publisher={Elsevier}
}
@inproceedings{martinez2020lipreading,
  title={Lipreading using temporal convolutional networks},
  author={Martinez, Brais and Ma, Pingchuan and Petridis, Stavros and Pantic, Maja},
  booktitle={ICASSP 2020-2020 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={6319--6323},
  year={2020},
  organization={IEEE}
}
@article{el2020ensemble,
  title={An ensemble method of full wavelet packet transform and neural network for short term electrical load forecasting},
  author={El-Hendawi, Mohamed and Wang, Zhanle},
  journal={Electric Power Systems Research},
  volume={182},
  pages={106265},
  year={2020},
  publisher={Elsevier}
}
@article{heidari2020ant,
  title={Ant lion optimizer: theory, literature review, and application in multi-layer perceptron neural networks},
  author={Heidari, Ali Asghar and Faris, Hossam and Mirjalili, Seyedali and Aljarah, Ibrahim and Mafarja, Majdi},
  journal={Nature-Inspired Optimizers: Theories, Literature Reviews and Applications},
  pages={23--46},
  year={2020},
  publisher={Springer}
}
@article{bouktif2018optimal,
  title={Optimal deep learning lstm model for electric load forecasting using feature selection and genetic algorithm: Comparison with machine learning approaches},
  author={Bouktif, Salah and Fiaz, Ali and Ouni, Ali and Serhani, Mohamed Adel},
  journal={Energies},
  number={7},
  pages={1636},
  year={2018},
  publisher={MDPI}
}
@article{abdel2019accurate,
  title={Accurate photovoltaic power forecasting models using deep LSTM-RNN},
  author={Abdel-Nasser, Mohamed and Mahmoud, Karar},
  journal={Neural computing and applications},
  volume={31},
  pages={2727--2740},
  year={2019},
  publisher={Springer}
}
@article{alhussein2020hybrid,
  title={Hybrid CNN-LSTM model for short-term individual household load forecasting},
  author={Alhussein, Musaed and Aurangzeb, Khursheed and Haider, Syed Irtaza},
  journal={Ieee Access},
  volume={8},
  pages={180544--180557},
  year={2020},
  publisher={IEEE}
}
@inproceedings{taik2020electrical,
  title={Electrical load forecasting using edge computing and federated learning},
  author={Ta{\"\i}k, Afaf and Cherkaoui, Soumaya},
  booktitle={ICC 2020-2020 IEEE international conference on communications (ICC)},
  pages={1--6},
  year={2020},
  organization={IEEE}
}
@article{tavakolian2023hospital,
  title={Hospital Readmission and Length-of-Stay Prediction Using an Optimized Hybrid Deep Model},
  author={Tavakolian, Alireza and Rezaee, Alireza and Hajati, Farshid and Uddin, Shahadat},
  journal={Future Internet},
  volume={15},
  number={9},
  pages={304},
  year={2023},
  publisher={MDPI}
}
@article{rafi2021short,
  title={A short-term load forecasting method using integrated CNN and LSTM network},
  author={Rafi, Shafiul Hasan and Deeba, Shohana Rahman and Hossain, Eklas and others},
  journal={IEEE Access},
  volume={9},
  pages={32436--32448},
  year={2021},
  publisher={IEEE}
}
@inproceedings{joga2021performance,
  title={Performance study of various machine learning classifiers for arc fault detection in AC microgrid},
  author={Joga, S Ramana Kumar and Sinha, Pampa and Maharana, Manoj Kumar},
  booktitle={IOP Conference Series: Materials Science and Engineering},
  volume={1131},
  number={1},
  pages={012012},
  year={2021},
  organization={IOP Publishing}
}
@article{wang2023fast,
  title={Fast SVM classifier for large-scale classification problems},
  author={Wang, Huajun and Li, Genghui and Wang, Zhenkun},
  journal={Information Sciences},
  volume={642},
  pages={119136},
  year={2023},
  publisher={Elsevier}
}
@article{ukey2023survey,
  title={Survey on exact knn queries over high-dimensional data space},
  author={Ukey, Nimish and Yang, Zhengyi and Li, Binghao and Zhang, Guangjian and Hu, Yiheng and Zhang, Wenjie},
  journal={Sensors},
  volume={23},
  number={2},
  pages={629},
  year={2023},
  publisher={MDPI}
}
@article{li2022area,
  title={The area prediction of western North Pacific Subtropical High in summer based on Gaussian Naive Bayes},
  author={Li, Deqian and Hu, Shujuan and He, Wenping and Zhou, Bingqian and Peng, Jianjun and Wang, Kai},
  journal={Climate Dynamics},
  volume={59},
  number={11-12},
  pages={3193--3210},
  year={2022},
  publisher={Springer}
}
@incollection{james2023tree,
  title={Tree-based methods},
  author={James, Gareth and Witten, Daniela and Hastie, Trevor and Tibshirani, Robert and Taylor, Jonathan},
  booktitle={An Introduction to Statistical Learning: with Applications in Python},
  pages={331--366},
  year={2023},
  publisher={Springer}
}
@article{baloch2021intelligent,
  title={An intelligent data mining-based fault detection and classification strategy for microgrid},
  author={Baloch, Shazia and Muhammad, Mannan Saeed},
  journal={IEEE Access},
  volume={9},
  pages={22470--22479},
  year={2021},
  publisher={IEEE}
}
@article{rangel2023optimisation,
  title={An optimisation tool for minimising fuel consumption, costs and emissions from Diesel-PV-Battery hybrid microgrids},
  author={Rangel, Nina and Li, Hu and Aristidou, Petros},
  journal={Applied Energy},
  volume={335},
  pages={120748},
  year={2023},
  publisher={Elsevier}
}
@article{kiranyaz20211d,
  title={1D convolutional neural networks and applications: A survey},
  author={Kiranyaz, Serkan and Avci, Onur and Abdeljaber, Osama and Ince, Turker and Gabbouj, Moncef and Inman, Daniel J},
  journal={Mechanical systems and signal processing},
  volume={151},
  pages={107398},
  year={2021},
  publisher={Elsevier}
}
@article{qian2023fault,
  title={Fault diagnosis based on gated recurrent unit network with attention mechanism and transfer learning under few samples in nuclear power plants},
  author={Qian, Gensheng and Liu, Jingquan},
  journal={Progress in Nuclear Energy},
  volume={155},
  pages={104502},
  year={2023},
  publisher={Elsevier}
}
@article{li2023deep,
  title={Deep learning attention mechanism in medical image analysis: Basics and beyonds},
  author={Li, Xiang and Li, Minglei and Yan, Pengfei and Li, Guanyi and Jiang, Yuchen and Luo, Hao and Yin, Shen},
  journal={International Journal of Network Dynamics and Intelligence},
  pages={93--116},
  year={2023}
}
@article{yan2019stat,
  title={STAT: Spatial-temporal attention mechanism for video captioning},
  author={Yan, Chenggang and Tu, Yunbin and Wang, Xingzheng and Zhang, Yongbing and Hao, Xinhong and Zhang, Yongdong and Dai, Qionghai},
  journal={IEEE transactions on multimedia},
  volume={22},
  number={1},
  pages={229--241},
  year={2019},
  publisher={IEEE}
}
@article{tavakolian2022source,
  title={Source code for optimized parallel inception: A fast COVID-19 screening software},
  author={Tavakolian, Alireza and Hajati, Farshid and Rezaee, Alireza and Fasakhodi, Amirhossein Oliaei and Uddin, Shahadat},
  journal={Software Impacts},
  volume={13},
  pages={100337},
  year={2022},
  publisher={Elsevier}
}
@article{moustafa2023predicting,
  title={Predicting characteristics of dissimilar laser welded polymeric joints using a multi-layer perceptrons model coupled with archimedes optimizer},
  author={Moustafa, Essam B and Elsheikh, Ammar},
  journal={Polymers},
  volume={15},
  number={1},
  pages={233},
  year={2023},
  publisher={MDPI}
}
@inproceedings{guo2003knn,
  title={KNN model-based approach in classification},
  author={Guo, Gongde and Wang, Hui and Bell, David and Bi, Yaxin and Greer, Kieran},
  booktitle={On The Move to Meaningful Internet Systems 2003: CoopIS, DOA, and ODBASE: OTM Confederated International Conferences, CoopIS, DOA, and ODBASE 2003, Catania, Sicily, Italy, November 3-7, 2003. Proceedings},
  pages={986--996},
  year={2003},
  organization={Springer}
}
@article{bouktif2018optimal,
  title={Optimal deep learning lstm model for electric load forecasting using feature selection and genetic algorithm: Comparison with machine learning approaches},
  author={Bouktif, Salah and Fiaz, Ali and Ouni, Ali and Serhani, Mohamed Adel},
  journal={Energies},
  volume={11},
  number={7},
  pages={1636},
  year={2018},
  publisher={MDPI}
}
@article{li2023deep,
  title={Deep learning attention mechanism in medical image analysis: Basics and beyonds},
  author={Li, Xiang and Li, Minglei and Yan, Pengfei and Li, Guanyi and Jiang, Yuchen and Luo, Hao and Yin, Shen},
  journal={International Journal of Network Dynamics and Intelligence},
  pages={93--116},
  year={2023}
}
@article{goudjil2018novel,
  title={A novel active learning method using SVM for text classification},
  author={Goudjil, Mohamed and Koudil, Mouloud and Bedda, Mouldi and Ghoggali, Noureddine},
  journal={International Journal of Automation and Computing},
  volume={15},
  pages={290--298},
  year={2018},
  publisher={Springer}
}
@article{charbuty2021classification,
  title={Classification based on decision tree algorithm for machine learning},
  author={Charbuty, Bahzad and Abdulazeez, Adnan},
  journal={Journal of Applied Science and Technology Trends},
  volume={2},
  number={01},
  pages={20--28},
  year={2021}
}
@article{guo2022attention,
  title={Attention mechanisms in computer vision: A survey},
  author={Guo, Meng-Hao and Xu, Tian-Xing and Liu, Jiang-Jiang and Liu, Zheng-Ning and Jiang, Peng-Tao and Mu, Tai-Jiang and Zhang, Song-Hai and Martin, Ralph R and Cheng, Ming-Ming and Hu, Shi-Min},
  journal={Computational visual media},
  volume={8},
  number={3},
  pages={331--368},
  year={2022},
  publisher={Springer}
}
@article{kattenborn2021review,
  title={Review on Convolutional Neural Networks (CNN) in vegetation remote sensing},
  author={Kattenborn, Teja and Leitloff, Jens and Schiefer, Felix and Hinz, Stefan},
  journal={ISPRS journal of photogrammetry and remote sensing},
  volume={173},
  pages={24--49},
  year={2021},
  publisher={Elsevier}
}
@article{sharma2022comprehensive,
  title={A comprehensive report on machine learning-based early detection of alzheimer's disease using multi-modal neuroimaging data},
  author={Sharma, Shallu and Mandal, Pravat Kumar},
  journal={ACM Computing Surveys (CSUR)},
  volume={55},
  number={2},
  pages={1--44},
  year={2022},
  publisher={ACM New York, NY}
}
@article{zhao2020xgb,
  title={XGB model: Research on evaporation duct height prediction based on XGBoost algorithm},
  author={Zhao, WP and Li, Jincai and Zhao, Jun and Zhao, Dandan and Lu, Jingze and Wang, Xiang},
  journal={Radioengineering},
  volume={29},
  number={1},
  pages={81--93},
  year={2020}
}
@article{aslam2021survey,
  title={A survey on deep learning methods for power load and renewable energy forecasting in smart microgrids},
  author={Aslam, Sheraz and Herodotou, Herodotos and Mohsin, Syed Muhammad and Javaid, Nadeem and Ashraf, Nouman and Aslam, Shahzad},
  journal={Renewable and Sustainable Energy Reviews},
  volume={144},
  pages={110992},
  year={2021},
  publisher={Elsevier}
}
@article{zampieri2021using,
  title={Using Bayesian methods to augment the interpretation of critical care trials. An overview of theory and example reanalysis of the alveolar recruitment for acute respiratory distress syndrome trial},
  author={Zampieri, Fernando G and Casey, Jonathan D and Shankar-Hari, Manu and Harrell Jr, Frank E and Harhay, Michael O},
  journal={American journal of respiratory and critical care medicine},
  volume={203},
  number={5},
  pages={543--552},
  year={2021},
  publisher={American Thoracic Society}
}
@article{cunningham2021k,
  title={k-Nearest neighbour classifiers-A Tutorial},
  author={Cunningham, Padraig and Delany, Sarah Jane},
  journal={ACM computing surveys (CSUR)},
  volume={54},
  number={6},
  pages={1--25},
  year={2021},
  publisher={ACM New York, NY, USA}
}
@inproceedings{abdelgawad2019comprehensive,
  title={A comprehensive review on microgrid architectures for distributed generation},
  author={Abdelgawad, Haytham and Sood, Vijay K},
  booktitle={2019 IEEE electrical power and energy conference (EPEC)},
  pages={1--8},
  year={2019},
  organization={IEEE}
}
@article{raza2015review,
  title={A review on artificial intelligence based load demand forecasting techniques for smart grid and buildings},
  author={Raza, Muhammad Qamar and Khosravi, Abbas},
  journal={Renewable and Sustainable Energy Reviews},
  volume={50},
  pages={1352--1372},
  year={2015},
  publisher={Elsevier}
}
@article{gust2021strategies,
  title={Strategies for microgrid operation under real-world conditions},
  author={Gust, Gunther and Brandt, Tobias and Mashayekh, Salman and Heleno, Miguel and DeForest, Nicholas and Stadler, Michael and Neumann, Dirk},
  journal={European Journal of Operational Research},
  volume={292},
  number={1},
  pages={339--352},
  year={2021},
  publisher={Elsevier}
}
@article{ibrahim2022machine,
  title={Machine learning for short-term load forecasting in smart grids},
  author={Ibrahim, Bibi and Rabelo, Luis and Gutierrez-Franco, Edgar and Clavijo-Buritica, Nicolas},
  journal={Energies},
  volume={15},
  number={21},
  pages={8079},
  year={2022},
  publisher={MDPI}
}
@inproceedings{navada2011overview,
  title={Overview of use of decision tree algorithms in machine learning},
  author={Navada, Arundhati and Ansari, Aamir Nizam and Patil, Siddharth and Sonkamble, Balwant A},
  booktitle={2011 IEEE control and system graduate research colloquium},
  pages={37--42},
  year={2011},
  organization={IEEE}
}
@article{sabzehgar2020solar,
  title={Solar power forecast for a residential smart microgrid based on numerical weather predictions using artificial intelligence methods},
  author={Sabzehgar, Reza and Amirhosseini, Diba Zia and Rasouli, Mohammad},
  journal={Journal of Building Engineering},
  volume={32},
  pages={101629},
  year={2020},
  publisher={Elsevier}
}
@article{damacharlacovid,
  title={TLU-Net: A Deep Learning Approach for Automatic Steel Surface Defect Detection},
  author={Damacharla, Praveen and Rao M. V., Achuth and Ringenberg, Jordan and Javaid, Ahmad},
  journal={2021 International Conference on Applied Artificial Intelligence (ICAPAI)}, 
  year={2021},
  volume={},
  number={},
  pages={1-6},
  doi={10.1109/ICAPAI49758.2021.9462060}
}

@INPROCEEDINGS{10590520,
  author={Damacharla, Praveen and Rajabalipanah, Hamid and Fakheri, Mohammad Hosein},
  booktitle={2023 International Conference on Computational Science and Computational Intelligence (CSCI)}, 
  title={LSTM-CNN Network for Audio Signature Analysis in Noisy Environments}, 
  year={Dec. 13-15, 2023},
  location={Las Vagas, USA},
  pages={78-82},
  doi={10.1109/CSCI62032.2023.00019}
}

@INPROCEEDINGS{SahuA2024,
  author={Abhishek Sahu, and Peter H. Aaen, and Praveen Damacharla},
  booktitle={2024 IEEE Texas Symposium on Wireless \& Micrwowave Circuits and Systems}, 
  title={An Automated Machine Learning Approach to Inkjet Printed Component Analysis: A Step Toward Smart Additive Manufacturing}, 
  year={April 3 - 4th, 2024},
  location={ Waco, USA},
  pages={1-6},
}


@article{suresh2020microgrid,
  title={Microgrid energy management system with embedded deep learning forecaster and combined optimizer},
  author={Suresh, Vishnu and Janik, Przemyslaw and Guerrero, Josep M and Leonowicz, Zbigniew and Sikorski, Tomasz},
  journal={IEEE Access},
  volume={8},
  pages={202225--202239},
  year={2020},
  publisher={IEEE}
}
@article{chen2023short,
  title={Short-term load forecasting and associated weather variables prediction using ResNet-LSTM based deep learning},
  author={Chen, Xinfang and Chen, Weiran and Dinavahi, Venkata and Liu, Yiqing and Feng, Jilin},
  journal={IEEE Access},
  volume={11},
  pages={5393--5405},
  year={2023},
  publisher={IEEE}
}
@article{hosseini2023privacy,
  title={Privacy-preserving federated learning: Application to behind-the-meter solar photovoltaic generation forecasting},
  author={Hosseini, Paniz and Taheri, Saman and Akhavan, Javid and Razban, Ali},
  journal={Energy Conversion and Management},
  volume={283},
  pages={116900},
  year={2023},
  publisher={Elsevier}
}
@article{awad2015support,
  title={Support vector machines for classification},
  author={Awad, Mariette and Khanna, Rahul and Awad, Mariette and Khanna, Rahul},
  journal={Efficient learning machines: Theories, concepts, and applications for engineers and system designers},
  pages={39--66},
  year={2015},
  publisher={Springer}
}






